MINED: Probing and Updating with Multimodal Time-Sensitive Knowledge for Large Multimodal Models

Large Multimodal Models (LMMs) encode rich factual knowledge via cross-modal pre-training, yet their static representations struggle to maintain an accurate understanding of time-sensitive factual knowledge. Existing benchmarks remain constrained by static designs, inadequately evaluating LMMs' ability to understand time-sensitive knowledge. To address this gap, we propose MINED, a comprehensive benchmark that evaluates temporal awareness along 6 key dimensions and 11 challenging tasks: cognition, awareness, trustworthiness, understanding, reasoning, and robustness. MINED is constructed from Wikipedia by two professional annotators, containing 2,104 time-sensitive knowledge samples spanning six knowledge types. Evaluating 15 widely used LMMs on MINED shows that Gemini-2.5-Pro achieves the highest average CEM score of 63.07, while most open-source LMMs still lack time understanding ability. Meanwhile, LMMs perform best on organization knowledge, whereas their performance is weakest on sport. To address these challenges, we investigate the feasibility of updating time-sensitive knowledge in LMMs through knowledge editing methods and observe that LMMs can effectively update knowledge via knowledge editing methods in single editing scenarios.

==> section/resubmission.tex <==

\definecolor{backred}{RGB}{255, 190, 190}
\definecolor{backblue}{RGB}{210, 230, 250}
\definecolor{verylightgray}{gray}{0.95} 

\definecolor{lightdarkred}{rgb}{0.9, 0.3, 0.4} % 自定义稍微亮一点的红色
\definecolor{brightorange}{rgb}{1.0, 0.5, 0.0}

\definecolor{brightpurple}{rgb}{0.5, 0.0, 0.8}
\newcommand{\cm}[2]{\noindent[#1] \textbf{#2}}

% 定义审稿人快捷命令
\newcommand{\rvone}{\textcolor{blue}{\textbf{R1}}}
\newcommand{\rvtwo}{\textcolor{magenta}{\textbf{R2}}}
\newcommand{\rvthree}{\textcolor{brightorange}{\textbf{R3}}}


\section*{Resubmission Report}



\noindent We appreciate the reviewers \textcolor{blue}{\textbf{yxFe}}(\textcolor{blue}{\textbf{R1}}), \textcolor{magenta}{\textbf{sriw}}(\textcolor{magenta}{\textbf{R2}}), \textcolor{brightorange}{\textbf{YYZ6}}(\textcolor{brightorange}{\textbf{R3}}) for their previous insightful feedback. In this resubmission, we provide \textbf{detailed clarifications for each previous concern} raised by the reviewers below to facilitate the review work.

\noindent \textcolor{brightpurple}{\textbf{General Response.}} In this resubmission, we restructure the entire work by recollecting the dataset and redesigning the evaluation dimensions, through which we propose \dataset, a comprehensive benchmark that evaluates temporal awareness in LMMs across six key dimensions and eleven challenging tasks while investigating knowledge editing for updating time-sensitive knowledge.




\cm{\rvone,\rvthree}{\dataset’s Evolvability.} Regarding previous concerns about the dynamic nature of \dataset, we provide a detailed pipeline in Appendix~\ref{appendix:benchmark_Evolvability} to demonstrate its evolvability, which enables easy version updates and provides a clear framework for future researchers to follow.


\cm{\rvone,\rvthree}{\dataset’s Evaluation Metrics.} To address concerns regarding evaluation standardization, the results in Section~\ref{sec:main_result} and Table~\ref{table:main_results_cem} utilize the widely recognized Cover Exact Match metric, with the formula detailed in Section~\ref{sec:Setup}. Additionally, in Exploration 3 of Section~\ref{sec:Exploratory}, we apply a fine-grained classification for Time-Agnostic tasks: \en{If any output contains the most up-to-date value from the attribute list $A$, it is labeled as \textbf{Latest}. If none includes the latest value but at least one contains an outdated answer, it is marked as \textbf{Outdated}. All other cases are categorized as \textbf{Irrelevant}.}

Furthermore, we introduce F1-Score and LLM as judge in Sections~\ref{appendix:metric_f1} and~\ref{appendix:metric_llm} for a more comprehensive evaluation, observing that while numerical results vary across metrics, the overall trends remain consistent, which confirms the reliability of our experimental conclusions.


\cm{\rvone}{A more rigorous matching process.} To address reviewers' concerns regarding the rigor of the answer matching process—specifically the oversight of entity aliases—we enhance our evaluation framework beyond the Cover Exact Match metric used in Section~\ref{sec:main_result}. While Exact Match is restricted to literal string overlap, we introduce F1-Score and LLM as judge in Appendices~\ref{appendix:metric_f1} and~\ref{appendix:metric_llm} to capture nuanced semantic variations. 

In particular, the LLM evaluator effectively recognizes aliases; for instance, as shown in the prompt details in Figure~\ref{fig:llm_judge_prompt}, it assigns a high score of 0.95 when the model predicts \en{Messi} against the ground truth \en{Lionel Messi}, demonstrating its robustness in semantic assessment.


\cm{\rvone}{A new approach for handling time-sensitive multimodal knowledge.} \ding{182} Core positioning of the work is to evaluate and to indicate directions for subsequent research: We focus on evaluating multimodal time-sensitive knowledge and propose \dataset, a multi-dimensional and comprehensive benchmark. Our work reveals the major deficiencies of existing LMMs in temporal awarenes. \ding{183} Knowledge editing serves as an exploratory tool: The purpose of introducing knowledge editing is to explore and validate its feasibility in updating time-sensitive knowledge of LMMs, rather than aiming to design novel knowledge editing methodologies.

\cm{\rvtwo}{Absence of clearly documented training data cutoff dates for the evaluated models.} Since the exact training data cutoff for LMMs is not directly accessible, we approximate it using the models' release dates. These dates are provided for reference in Tables~\ref{table:main_results_cem}, \ref{table:all_f1}, \ref{table:all_cem}, and \ref{table:gpt_eval}.

\cm{\rvtwo}{Clarifying the data construction process, collecting generalization images, and distinguishing them from the original images.} \ding{182} In our data construction process, we categorize the \dataset data into original and task-specific datasets. The original data, collected from Wikipedia by professional annotators across six domains, is formatted as the quadruple $(S, H, P, A)$ shown in Figure~\ref{fig:overview}; its collection pipeline is detailed in Appendix~\ref{appendix:original_construction_pipeline} and Figure~\ref{fig:Original_data_construction}. 

Task data is generated by transforming these quadruples through specific rules, with the construction of its six key dimensions—Cognition, Awareness, Trustworthiness, Understanding, Reasoning, and Robustness—elaborated in Sections~\ref{sec:Cognition},~\ref{sec:Awareness},~\ref{sec:Trustworthiness},~\ref{sec:Understanding},~\ref{sec:Reasoning},~\ref{sec:Robustness} and Appendix~\ref{appendix:task_construction_pipeline}.


\ding{183} In Figure~\ref{fig:Original_data_construction}, we clarify that generalization images are sourced from Google and matched with original images using cosine similarity.

\ding{184} Both generalization and original images depict the same entity and are semantically equivalent, differing only in the environmental context of the visuals. We introduce generalization images primarily to utilize Prompt Agreement (in Section~\ref{sec:Setup}), which helps mitigate uncertainty arising from prompt variations.


\ding{185} In Appendix~\ref{appendix:result_prompt_agreement} and Table~\ref{table:prompt_agreement_eval}, we discuss the impact of using prompt agreement on evaluation results. We find that while using generalization versus original images causes numerical fluctuations, these changes are minimal and remain within a normal, expected range.




\cm{\rvtwo}{Human validation details and quantification of dataset quality.} \ding{182} In Appendices~\ref{appendix:original_construction_pipeline}, \ref{appendix:task_construction_pipeline}, and Figure~\ref{fig:Original_data_construction}, we clarify our data construction pipeline and specify the manual verification steps. Furthermore, we discuss data quality in Appendix~\ref{appendix:data_quality} and include a human study to validate the reliability of our dataset.

\ding{183} In Appendix~\ref{appendix:Inter_Annotator_Agreement_Numebers} and Table~\ref{tab:kappa_agreement}, we provide Inter-Annotator Agreement numbers calculated via Cohen's Kappa for reference.


\cm{\rvthree}{Unique design elements for time-sensitive knowledge.} Our \dataset serves as a comprehensive benchmark evaluating temporal awareness in LMMs across six key dimensions,including Cognition, Awareness, Trustworthiness, Understanding, Reasoning, and Robustness and eleven challenging tasks, including Time-Agnostic, Timestamp-Aware, Temporal Interval-Aware, Future Misaligned Context, Past Misaligned Context, Past Unanswerable Date, Future Unanswerable Date, Implicit Temporal Concept, Ranking, Calculation, and Adversarial Temporal Error. We believe these unique design elements for time-sensitive knowledge highlight the comprehensiveness and distinctiveness of \dataset.


\cm{\rvthree}{Analysis of experimental results on time-sensitive knowledge.} Based on Section~\ref{sec:main_result} and Table~\ref{table:main_results_cem}, we present specific experimental findings for each of the six key dimensions,including Cognition, Awareness, Trustworthiness, Understanding, Reasoning, and Robustness to reveal the limitations of current LMMs in temporal knowledge evaluation, supported by illustrative cases in Figures~\ref{fig:ob1},~\ref{fig:ob2} ,~\ref{fig:ob3} ,~\ref{fig:ob4} ,~\ref{fig:ob5} and~\ref{fig:ob6}. Alongside an overall conclusion, we discuss Fine-grained Knowledge Types, Model Size, Temporal Distributions, and Error Analysis in Section~\ref{sec:Exploratory}, while exploring the impact of Foundation LLMs in Appendix~\ref{appendix:result_Foundation_LLM}. We believe these unique experimental insights provide valuable guidance for future research.





\cm{\rvthree}{Depth of analysis in knowledge editing experiments.} \ding{182} Core positioning of the work is to evaluate and to indicate directions for subsequent research: We focus on evaluating multimodal time-sensitive knowledge and propose \dataset, a multi-dimensional and comprehensive benchmark. Our work reveals the major deficiencies of existing LMMs in temporal awarenes. \ding{183} Knowledge editing serves as an exploratory tool: The purpose of introducing knowledge editing is to explore and validate its feasibility in updating time-sensitive knowledge of LMMs, rather than aiming to design novel knowledge editing methodologies. \ding{184} Speculation of catastrophic forgetting: We offer thoughts on catastrophic forgetting in lifelong editing. Knowledge editing methods typically use \textbf{a pipeline mode where they perform a single iteration on each editing sample until convergence before moving to the next}. This process leads to overfitting the current sample, which strongly interferes with the model weights and prevents consistency across multiple edits, thereby causing catastrophic forgetting of previously edited samples and original knowledge. In Appendix~\ref{appendix:ke_Analysis} and Table~\ref{tab:gap_analysis}, we conduct preliminary experiments to validate this hypothesis.


\cm{\rvthree}{Careful filling of the checklist.} In this submission, we complete every item in the checklist, with particular attention to the \textbf{\en{B Use Or Create Scientific Artifacts}}, to ensure the integrity of our research.

\cm{\rvthree}{Presentation of manuscript.} In this submission, we restructure the entire manuscript and adjust the dimensions of all tables and figures to ensure readability and effective interpretation. Furthermore, we reference all appendices within the main text to improve overall coherence and enable readers to locate supplementary information easily.




\noindent \textcolor{brightpurple}{\textbf{Report Summary.}} Below, we will summarize the improvements made to \dataset's work.

\noindent \textbf{1.Presentation.} We restructure the manuscript and redesign all tables and figures to improve the overall flow and readability of the manuscript.

\noindent \textbf{2.Design.} To highlight the uniqueness of \dataset regarding time-sensitive knowledge, we design six key dimensions,including Cognition, Awareness, Trustworthiness, Understanding, Reasoning, and Robustness and comprising eleven challenging tasks,including Time-Agnostic, Timestamp-Aware, Temporal Interval-Aware, Future Misaligned Context, Past Misaligned Context, Past Unanswerable Date, Future Unanswerable Date, Implicit Temporal Concept, Ranking, Calculation, and Adversarial Temporal Error.

\noindent \textbf{3.Clarification.}  \ding{182} We clarify the data construction pipeline of \dataset in Section~\ref{sec:Benchmark_Construction} and Appendix~\ref{appendix:benchmark_details}.   \ding{183} In the restructured manuscript, we clarify the positioning and contributions of our work to facilitate better understanding for future readers.

\noindent \textbf{4.Analysis.} In Sections~\ref{sec:main_result} and~\ref{sec:Exploratory}, we analyze time-sensitive knowledge, while in Section~\ref{sec:challenges}, we evaluate and discuss the feasibility of using knowledge editing methods to update multimodal time-sensitive knowledge.



